Learning without Recall by Random Walks on Directed Graphs

We consider a network of agents that aim to learn some unknown state of the world using private observations and exchange of beliefs. At each time, agents observe private signals generated based on the true unknown state. Each agent might not be able to distinguish the true state based only on her private observations. This occurs when some other states are observationally equivalent to the true state from the agent's perspective. To overcome this shortcoming, agents must communicate with each other to benefit from local observations. We propose a model where each agent selects one of her neighbors randomly at each time. Then, she refines her opinion using her private signal and the prior of that particular neighbor. The proposed rule can be thought of as a Bayesian agent who cannot recall the priors based on which other agents make inferences. This learning without recall approach preserves some aspects of the Bayesian inference while being computationally tractable. By establishing a correspondence with a random walk on the network graph, we prove that under the described protocol, agents learn the truth exponentially fast in the almost sure sense. The asymptotic rate is expressed as the sum of the relative entropies between the signal structures of every agent weighted by the stationary distribution of the random walk.

==> oldSignalStructureModel.tex <==
and at any given time $t$, each agent makes a signal observation that is independent of the rest of the agents. In particular, for $t \in \mathbb{W}$ and $\hat{\theta} \in \Theta$ both fixed, let $\mathcal{L}(\cdot \mid \hat{\theta})$ denote the joint law for the random vector $(\mathbf{s}_{1,t},\ldots,\mathbf{s}_{n,t})$, then $\mathcal{L}( \mathord{\cdot} \mid \hat{\theta})$ does not depend on $t$, and it factors
\begin{align}
{\mathcal{L}}( \mathord{\cdot} \mid \hat{\theta}) = \prod_{i\in[n]}\ell_i(\mathord{\cdot}\mid \hat{\theta}),
\label{eq:joint_law}
\end{align} as the product probability measure on the product space $\prod_{i\in[n]}\mathcal{S}_{i}$. The signal structures and the joint law given in \eqref{eq:joint_law}, as well as the common prior $\nu(\mathord{\cdot})$ and their corresponding sample spaces $\prod_{i \in [n]}\mathcal{S}_i$ and $\Theta$ are common knowledge amongst all the agents. The assumption of common knowledge in the case of fully rational (Bayesian) agents implies that given the same observations of one another's beliefs or private signals distinct agents would make identical inferences; in the sense that starting form the same belief about the unknown $\boldsymbol\theta$, their updated beliefs given the same observations, would be the same.
